Diversity-By-Design for Dependable and Secure Cyber-Physical Systems: A Survey

Diversity-based security approaches have been studied for several decades since the 1970's. The concept of diversity-by-design emerged in the 1980's and, since then, diversity-based system design research has been explored to build more secure and dependable systems. In this work, we are particularly interested in providing an in-depth, comprehensive survey of existing diversity-based approaches, insights, and future work directions for those who want to conduct research on developing secure and dependable cyber-physical systems (CPSs) using diversity as a system design feature. To be specific, this survey paper provides: (i) The common concept of diversity based on a multidisciplinary study of diversity from nine different fields along with the historical evolution of diversity-by-design for security; (ii) The design principles of diversity-based approaches; (iii) The key benefits and caveats of using diversity-by-design; (iv) The key concerns of CPS environments in introducing diversity-by-design; (v) A variety of existing diversity-based approaches based on five different classifications; (vi) The types of attacks mitigated by existing diversity-based approaches; (vii) The overall trends of evaluation methodologies used in diversity-based approaches, in terms of metrics, datasets, and testbeds; and (viii) The insights, lessons, and gaps identified from this extensive survey.

==> figs/multi_layer_CPS.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% %
% % Welcome to Overleaf --- just edit your LaTeX on the left,
% % and we'll compile it for you on the right. If you open the
% % 'Share' menu, you can invite other users to edit at the same
% % time. See www.overleaf.com/learn for more info. Enjoy!
% %
% % Note: you can export the pdf to see the result at full
% % resolution.
% %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \documentclass{article}
% \usepackage{tikz}
% %%%<
% \usepackage{verbatim}
% \usepackage[active,tightpage]{preview}
% \PreviewEnvironment{tikzpicture}
% \setlength\PreviewBorder{10pt}%
% %%%>
% \begin{comment}
% :Title: Work breakdown structures aka WBS diagrams
% :Tags: Charts;Diagrams;Trees
% :Author: Gonzalo Medina
% :Slug: work-breakdown-structure

% A work breakdown structure (WBS) diagram, is for decomposing a task into smaller parts, which helps organizing and performing. This example diagram shows possible tasks for designing a TikZ diagram. The basis is a tree, nodes were addes below its child nodes. It was originally posted by Gonzalo Medina as TeX.SE (http://tex.stackexchange.com/q/81809/213), modified by Stefan Kottwitz.
% \end{comment}
% \usetikzlibrary{arrows,shapes,positioning,shadows,trees}

% % \tikzset{
% %   basic/.style  = {draw, text width=2cm, drop shadow, font=\sffamily, rectangle},
% %   root/.style   = {basic, rounded corners=2pt, thin, align=center,
% %                   fill=green!30},
% %   level 2/.style = {basic, rounded corners=6pt, thin,align=center, fill=green!60,
% %                   text width=4em},
% %   level 3/.style = {basic, thin, align=left, fill=pink!60, text width=3.5em}
% % }

% \begin{document}
\begin{tikzpicture}[
    basic/.style  = {draw, text width=4cm, rectangle, font=\small},
    root/.style   = {basic, rounded corners=2pt, thin, align=center, fill=green!60},
    level 1/.style={basic, rounded corners=6pt, thin,align=center, fill=green!30, text width=6em, sibling distance=28mm},
    level 2/.style = {basic, rounded corners=6pt, thin, align=center, fill=yellow!60, text width=5em, sibling distance=28mm},
    edge from parent/.style={->,draw},
    level 3/.style = {basic, rounded corners=6pt, thin, align=center, fill=pink!60, text width=5em},
    level distance=3em
  ]
  

% root of the the initial tree, level 1
\node[root] {LAYERS}
% The first level, as children of the initial tree
  child {node[level 1] (c1) {Physical Environment}}
  child {node[level 1] (c2) {Network Diversity}}
  child {node[level 1] (c3) {Hardware}}
  child {node[level 1] (c4) {Software}}
  child {node[level 1] (c5) {Human-Related Factors}};

% The Third level, relatively positioned nodes
\begin{scope}[every node/.style={level 3}]
\node [below of = c2, xshift=15pt,yshift=-5pt] (c21) {Diversity Generation};
\node [below of = c21, yshift=-10pt] (c22) {Diversity Quantification};
\node [below of = c22, yshift=-15pt] (c23) {Diversity Deployment};
\node [below of = c3, xshift=15pt] (c31) {Sensors and Actuators};
\node [below of = c31, yshift=-10pt] (c32) {Comm. Modules};
\node [below of = c32, yshift=-10pt] (c33) {Embedded Devices};
\node [below of = c4, xshift=15pt] (c41) {Operating System};
\node [below of = c41, yshift=5pt] (c42) {Firewall};
\node [below of = c42, yshift=10pt] (c43) {IDS};
\node [below of = c43] (c44) {Malware Detection (\ref{subsubsec:malware})};
\node [below of = c44, yshift=-10pt] (c45) {Cryptographic Authentication};
\node [below of = c45, yshift=-15pt] (c46) {Instruction Diversification};
\node [below of = c46, yshift=-10pt] (c47) {Code Obfuscation};
\node [below of = c47, yshift=-5pt] (c48) {Control-Flow};

\end{scope}

% lines from each level 1 node to every one of its "children"
\foreach \value in {1,...,3}
  \draw[->] (c2.208) |- (c2\value.west);

\foreach \value in {1,...,3}
  \draw[->] (c3.195) |- (c3\value.west);
  
\foreach \value in {1,...,8}
  \draw[->] (c4.195) |- (c4\value.west);

\end{tikzpicture}
% \end{document}
